PuzzlePlex: Benchmarking Foundation Models on Reasoning and Planning with Puzzles

This work investigates the reasoning and planning capabilities of foundation models and their scalability in complex, dynamic environments. We introduce PuzzlePlex, a benchmark designed to assess these capabilities through a diverse set of puzzles. PuzzlePlex consists of 15 types of puzzles, including deterministic and stochastic games of varying difficulty, as well as single-player and two-player scenarios. The PuzzlePlex framework provides a comprehensive environment for each game, and supports extensibility to generate more challenging instances as foundation models evolve. Additionally, we implement customized game-playing strategies for comparison. Building on this benchmark, we develop fine-grained metrics to measure performance and conduct an in-depth analysis of frontier foundation models across two settings: instruction-based and code-based. Furthermore, we systematically investigate their scaling limits. Our findings show that reasoning models outperform others in instruction-based settings, while code-based execution presents greater challenges but offers a scalable and efficient alternative. PuzzlePlex enables targeted evaluation and guides future improvements in reasoning, planning, and generalization for foundation models.

==> figures/best_of_n.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{figures/Figure_3.png}
        \label{fig:line1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{figures/Figure_4.png}
        \label{fig:line2}
    \end{subfigure}
    \caption{Normalized score of models in Best-of-N (BoN) sampling}
    \label{fig:best_of_n}
\end{figure}


==> tables/ablation_analysis.tex <==
\begin{table}[ht]
% \centering
\begin{minipage}[t]{0.48\textwidth}
    \centering
    \small
    \captionsetup{font=small}
    \caption{}
    \addtolength{\tabcolsep}{-0.2em}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{lcccccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} &
    \multicolumn{2}{c}{\textbf{TidyTower}} &
    \multicolumn{2}{c}{\textbf{SudoKill}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    & \textbf{Easy} & \textbf{Normal} & \textbf{Easy} & \textbf{Normal} \\ 
    \midrule
    GPT-4.1 & 0.00 & 0.00 & 0.30 & 0.10 \\
    \noalign{\vskip 0.5ex}\hdashline\noalign{\vskip 0.5ex}
    \quad $w/$ 1-shot  & 0.00 & 0.00 & 0.10 & 0.10\\
    \noalign{\vskip 0.5ex}\hdashline\noalign{\vskip 0.5ex}
    \quad $w/$ ToT  & 0.60 & 0.80 & 0.30 & 0.10\\
    \noalign{\vskip 0.5ex}\hdashline\noalign{\vskip 0.5ex}
    \quad $w/o$ history & 1.00 & 0.90 & 0.20 & 0.00\\
    \noalign{\vskip 0.5ex}\hdashline\noalign{\vskip 0.5ex}
    \quad $w/$ legal candidates & 0.60 & 0.00 & 0.60 & 0.70 \\
    \midrule
    o4-mini & 0.00 & 0.00 & 0.40 & 0.20 \\
    \noalign{\vskip 0.5ex}\hdashline\noalign{\vskip 0.5ex}
    \quad $w/$ 1-shot & 0.00 & 0.00 & 0.50 & 0.20  \\
    \noalign{\vskip 0.5ex}\hdashline\noalign{\vskip 0.5ex}
    \quad $w/$ ToT & 0.80 & 0.70 & 0.40 & 0.40 \\
    \noalign{\vskip 0.5ex}\hdashline\noalign{\vskip 0.5ex}
    \quad $w/o$ history & 1.00 & 1.00 \\
    \noalign{\vskip 0.5ex}\hdashline\noalign{\vskip 0.5ex}
    \quad $w/$ legal candidates & 1.00 & 0.60 \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:ablation}
    \end{minipage}
\end{table}


==> tables/tmp_group.tex <==
-- single-det --
 [easy]
     custom → 1250.9 ±504.5
     gpt-4.1 → 1041.8 ±321.8
     o4-mini → 1094.9 ±549.8
     gemini-2.5-pro-preview-03-25 → 1082.1 ±494.9
     grok-3-mini-beta → 882.4 ±366.0
     deepseek-reasoner → 1146.6 ±445.8
     deepseek-chat → 980.2 ±60.4
     phi-4-multimodal-instruct → 819.8 ±294.0
     qwq → 1074.1 ±268.5
     llama → 863.3 ±381.6
     gemma → 858.8 ±397.7
     qwen → 905.2 ±349.7
 [normal]
     custom → 1229.9 ±529.1
     gpt-4.1 → 1042.5 ±321.4
     o4-mini → 1120.0 ±649.5
     gemini-2.5-pro-preview-03-25 → 1046.3 ±241.2
     grok-3-mini-beta → 911.1 ±254.8
     deepseek-reasoner → 1084.3 ±379.5
     deepseek-chat → 950.7 ±89.1
     phi-4-multimodal-instruct → 866.0 ±322.9
     qwq → 988.2 ±269.8
     llama → 891.9 ±266.0
     gemma → 918.3 ±217.5
     qwen → 950.7 ±282.0

-- two-det --
 [easy]
     custom → 1060.8 ±309.8
     gpt-4.1 → 1024.8 ±137.2
     o4-mini → 1165.7 ±96.0
     gemini-2.5-pro-preview-03-25 → 1145.0 ±64.3
     grok-3-mini-beta → 1145.9 ±190.1
     deepseek-reasoner → 1163.9 ±122.0
     deepseek-chat → 989.6 ±163.4
     phi-4-multimodal-instruct → 757.2 ±144.9
     qwq → 1160.0 ±111.5
     llama → 826.9 ±108.3
     gemma → 797.5 ±114.3
     qwen → 762.6 ±117.0
 [normal]
     custom → 1081.3 ±347.2
     gpt-4.1 → 1044.7 ±111.1
     o4-mini → 1156.4 ±100.3
     gemini-2.5-pro-preview-03-25 → 1117.8 ±136.7
     grok-3-mini-beta → 1120.6 ±225.1
     deepseek-reasoner → 1185.1 ±126.2
     deepseek-chat → 967.7 ±87.9
     phi-4-multimodal-instruct → 796.5 ±97.6
     qwq → 1122.9 ±84.4
     llama → 792.1 ±99.6
     gemma → 797.7 ±103.2
     qwen → 817.2 ±194.8


=== Combined All Elo Scores ===
     custom → 1134.6 ±126.4
     gpt-4.1 → 1037.5 ±53.1
     o4-mini → 1140.9 ±74.9
     gemini-2.5-pro-preview-03-25 → 1106.2 ±58.1
     grok-3-mini-beta → 1044.6 ±97.5
     deepseek-reasoner → 1152.4 ±63.2
     deepseek-chat → 973.7 ±42.7
     phi-4-multimodal-instruct → 801.6 ±55.8
     qwq → 1100.1 ±54.7
     llama → 835.0 ±52.9
     gemma → 831.7 ±55.8
     qwen → 841.7 ±73.0

==> tables/tmp_per_puzzle.tex <==

=== Per-Puzzle Elo Scores ===

TidyTowerPuzzle:
 [easy]
   TidyTowerCustomStrategy → 1481.3
   TidyTowerLLMStrategy:deepseek-chat → 956.2
   TidyTowerLLMStrategy:deepseek-reasoner → 956.2
   TidyTowerLLMStrategy:gemini-2.5-pro-preview-03-25 → 956.1
   TidyTowerLLMStrategy:gemma → 956.4
   TidyTowerLLMStrategy:gpt-4.1 → 956.1
   TidyTowerLLMStrategy:grok-3-mini-beta → 956.2
   TidyTowerLLMStrategy:llama → 956.3
   TidyTowerLLMStrategy:o4-mini → 956.1
   TidyTowerLLMStrategy:phi-4-multimodal-instruct → 956.3
   TidyTowerLLMStrategy:qwen → 956.4
   TidyTowerLLMStrategy:qwq → 956.3
 [normal]
   TidyTowerCustomStrategy → 1464.0
   TidyTowerLLMStrategy:deepseek-chat → 952.2
   TidyTowerLLMStrategy:deepseek-reasoner → 952.4
   TidyTowerLLMStrategy:gemini-2.5-pro-preview-03-25 → 952.7
   TidyTowerLLMStrategy:gemma → 951.8
   TidyTowerLLMStrategy:gpt-4.1 → 953.0
   TidyTowerLLMStrategy:grok-3-mini-beta → 952.5
   TidyTowerLLMStrategy:llama → 951.9
   TidyTowerLLMStrategy:o4-mini → 952.8
   TidyTowerLLMStrategy:phi-4-multimodal-instruct → 952.1
   TidyTowerLLMStrategy:qwen → 1012.7
   TidyTowerLLMStrategy:qwq → 952.0

OptimalTouringPuzzle:
 [easy]
   OptimalTouringCustomStrategy → 1098.1
   OptimalTouringLLMStrategy:deepseek-chat → 1004.8
   OptimalTouringLLMStrategy:deepseek-reasoner → 1312.6
   OptimalTouringLLMStrategy:gemini-2.5-pro-preview-03-25 → 1311.8
   OptimalTouringLLMStrategy:gemma → 674.1
   OptimalTouringLLMStrategy:gpt-4.1 → 1190.8
   OptimalTouringLLMStrategy:grok-3-mini-beta → 712.7
   OptimalTouringLLMStrategy:llama → 686.0
   OptimalTouringLLMStrategy:o4-mini → 1350.1
   OptimalTouringLLMStrategy:phi-4-multimodal-instruct → 744.4
   OptimalTouringLLMStrategy:qwen → 746.0
   OptimalTouringLLMStrategy:qwq → 1168.7
 [normal]
   OptimalTouringCustomStrategy → 1047.6
   OptimalTouringLLMStrategy:deepseek-chat → 914.1
   OptimalTouringLLMStrategy:deepseek-reasoner → 1251.6
   OptimalTouringLLMStrategy:gemini-2.5-pro-preview-03-25 → 1146.5
   OptimalTouringLLMStrategy:gemma → 819.0
   OptimalTouringLLMStrategy:gpt-4.1 → 1190.9
   OptimalTouringLLMStrategy:grok-3-mini-beta → 794.3
   OptimalTouringLLMStrategy:llama → 768.3
   OptimalTouringLLMStrategy:o4-mini → 1421.3
   OptimalTouringLLMStrategy:phi-4-multimodal-instruct → 716.5
   OptimalTouringLLMStrategy:qwen → 819.8
   OptimalTouringLLMStrategy:qwq → 1110.3

CountMaximalCocktailsPuzzle:
 [easy]
   CountMaximalCocktailsCustomStrategy → 1173.2
   CountMaximalCocktailsLLMStrategy:deepseek-chat → 979.7
   CountMaximalCocktailsLLMStrategy:deepseek-reasoner → 1170.9
   CountMaximalCocktailsLLMStrategy:gemini-2.5-pro-preview-03-25 → 978.3
   CountMaximalCocktailsLLMStrategy:gemma → 946.1
   CountMaximalCocktailsLLMStrategy:gpt-4.1 → 978.4
   CountMaximalCocktailsLLMStrategy:grok-3-mini-beta → 978.2
   CountMaximalCocktailsLLMStrategy:llama → 947.5
   CountMaximalCocktailsLLMStrategy:o4-mini → 978.4
   CountMaximalCocktailsLLMStrategy:phi-4-multimodal-instruct → 758.9
   CountMaximalCocktailsLLMStrategy:qwen → 1013.2
   CountMaximalCocktailsLLMStrategy:qwq → 1097.2
 [normal]
   CountMaximalCocktailsCustomStrategy → 1178.2
   CountMaximalCocktailsLLMStrategy:deepseek-chat → 985.8
   CountMaximalCocktailsLLMStrategy:deepseek-reasoner → 1048.8
   CountMaximalCocktailsLLMStrategy:gemini-2.5-pro-preview-03-25 → 1039.8
   CountMaximalCocktailsLLMStrategy:gemma → 984.2
   CountMaximalCocktailsLLMStrategy:gpt-4.1 → 983.8
   CountMaximalCocktailsLLMStrategy:grok-3-mini-beta → 986.5
   CountMaximalCocktailsLLMStrategy:llama → 955.5
   CountMaximalCocktailsLLMStrategy:o4-mini → 985.8
   CountMaximalCocktailsLLMStrategy:phi-4-multimodal-instruct → 929.4
   CountMaximalCocktailsLLMStrategy:qwen → 1019.8
   CountMaximalCocktailsLLMStrategy:qwq → 902.4

CardNimPuzzle:
 [easy]
   CardNimCustomStrategy → 688.9
   CardNimLLMStrategy:deepseek-chat → 1042.0
   CardNimLLMStrategy:deepseek-reasoner → 1245.8
   CardNimLLMStrategy:gemini-2.5-pro-preview-03-25 → 1201.7
   CardNimLLMStrategy:gemma → 890.8
   CardNimLLMStrategy:gpt-4.1 → 984.1
   CardNimLLMStrategy:grok-3-mini-beta → 1340.8
   CardNimLLMStrategy:llama → 839.8
   CardNimLLMStrategy:o4-mini → 1206.8
   CardNimLLMStrategy:phi-4-multimodal-instruct → 627.6
   CardNimLLMStrategy:qwen → 679.4
   CardNimLLMStrategy:qwq → 1252.2
 [normal]
   CardNimCustomStrategy → 697.6
   CardNimLLMStrategy:deepseek-chat → 1002.4
   CardNimLLMStrategy:deepseek-reasoner → 1265.2
   CardNimLLMStrategy:gemini-2.5-pro-preview-03-25 → 1221.1
   CardNimLLMStrategy:gemma → 752.7
   CardNimLLMStrategy:gpt-4.1 → 1084.2
   CardNimLLMStrategy:grok-3-mini-beta → 1313.8
   CardNimLLMStrategy:llama → 847.7
   CardNimLLMStrategy:o4-mini → 1153.9
   CardNimLLMStrategy:phi-4-multimodal-instruct → 680.9
   CardNimLLMStrategy:qwen → 789.9
   CardNimLLMStrategy:qwq → 1190.7

SudoKillPuzzle:
 [easy]
   SudoKillCustomStrategy → 1155.1
   SudoKillLLMStrategy:deepseek-chat → 1198.3
   SudoKillLLMStrategy:deepseek-reasoner → 1050.3
   SudoKillLLMStrategy:gemini-2.5-pro-preview-03-25 → 1160.3
   SudoKillLLMStrategy:gemma → 662.3
   SudoKillLLMStrategy:gpt-4.1 → 1071.9
   SudoKillLLMStrategy:grok-3-mini-beta → 1216.0
   SudoKillLLMStrategy:llama → 789.3
   SudoKillLLMStrategy:o4-mini → 1149.5
   SudoKillLLMStrategy:phi-4-multimodal-instruct → 709.1
   SudoKillLLMStrategy:qwen → 705.5
   SudoKillLLMStrategy:qwq → 1132.3
 [normal]
   SudoKillCustomStrategy → 1355.5
   SudoKillLLMStrategy:deepseek-chat → 964.0
   SudoKillLLMStrategy:deepseek-reasoner → 1266.1
   SudoKillLLMStrategy:gemini-2.5-pro-preview-03-25 → 1090.6
   SudoKillLLMStrategy:gemma → 771.3
   SudoKillLLMStrategy:gpt-4.1 → 1033.7
   SudoKillLLMStrategy:grok-3-mini-beta → 1260.2
   SudoKillLLMStrategy:llama → 653.9
   SudoKillLLMStrategy:o4-mini → 1048.4
   SudoKillLLMStrategy:phi-4-multimodal-instruct → 780.3
   SudoKillLLMStrategy:qwen → 659.5
   SudoKillLLMStrategy:qwq → 1116.5

MaxMaximalCocktailsPuzzle:
 [easy]
   MaxMaximalCocktailsCustomStrategy → 1274.6
   MaxMaximalCocktailsLLMStrategy:deepseek-chat → 898.5
   MaxMaximalCocktailsLLMStrategy:deepseek-reasoner → 1110.9
   MaxMaximalCocktailsLLMStrategy:gemini-2.5-pro-preview-03-25 → 1063.4
   MaxMaximalCocktailsLLMStrategy:gemma → 875.7
   MaxMaximalCocktailsLLMStrategy:gpt-4.1 → 999.3
   MaxMaximalCocktailsLLMStrategy:grok-3-mini-beta → 935.0
   MaxMaximalCocktailsLLMStrategy:llama → 971.4
   MaxMaximalCocktailsLLMStrategy:o4-mini → 1039.1
   MaxMaximalCocktailsLLMStrategy:phi-4-multimodal-instruct → 937.6
   MaxMaximalCocktailsLLMStrategy:qwen → 873.3
   MaxMaximalCocktailsLLMStrategy:qwq → 1021.2
 [normal]
   MaxMaximalCocktailsCustomStrategy → 1106.5
   MaxMaximalCocktailsLLMStrategy:deepseek-chat → 1012.8
   MaxMaximalCocktailsLLMStrategy:deepseek-reasoner → 1025.3
   MaxMaximalCocktailsLLMStrategy:gemini-2.5-pro-preview-03-25 → 1109.0
   MaxMaximalCocktailsLLMStrategy:gemma → 936.1
   MaxMaximalCocktailsLLMStrategy:gpt-4.1 → 990.0
   MaxMaximalCocktailsLLMStrategy:grok-3-mini-beta → 864.6
   MaxMaximalCocktailsLLMStrategy:llama → 847.8
   MaxMaximalCocktailsLLMStrategy:o4-mini → 1124.0
   MaxMaximalCocktailsLLMStrategy:phi-4-multimodal-instruct → 886.4
   MaxMaximalCocktailsLLMStrategy:qwen → 1081.2
   MaxMaximalCocktailsLLMStrategy:qwq → 1016.3

ExclusivityParticlesPuzzle:
 [easy]
   ExclusivityParticlesCustomStrategy → 1257.2
   ExclusivityParticlesLLMStrategy:deepseek-chat → 913.8
   ExclusivityParticlesLLMStrategy:deepseek-reasoner → 1126.8
   ExclusivityParticlesLLMStrategy:gemini-2.5-pro-preview-03-25 → 1166.5
   ExclusivityParticlesLLMStrategy:gemma → 771.4
   ExclusivityParticlesLLMStrategy:gpt-4.1 → 885.7
   ExclusivityParticlesLLMStrategy:grok-3-mini-beta → 1069.1
   ExclusivityParticlesLLMStrategy:llama → 786.8
   ExclusivityParticlesLLMStrategy:o4-mini → 1196.9
   ExclusivityParticlesLLMStrategy:phi-4-multimodal-instruct → 793.2
   ExclusivityParticlesLLMStrategy:qwen → 857.0
   ExclusivityParticlesLLMStrategy:qwq → 1175.4
 [normal]
   ExclusivityParticlesCustomStrategy → 1331.1
   ExclusivityParticlesLLMStrategy:deepseek-chat → 846.3
   ExclusivityParticlesLLMStrategy:deepseek-reasoner → 1146.8
   ExclusivityParticlesLLMStrategy:gemini-2.5-pro-preview-03-25 → 1216.1
   ExclusivityParticlesLLMStrategy:gemma → 806.1
   ExclusivityParticlesLLMStrategy:gpt-4.1 → 941.5
   ExclusivityParticlesLLMStrategy:grok-3-mini-beta → 1026.6
   ExclusivityParticlesLLMStrategy:llama → 811.6
   ExclusivityParticlesLLMStrategy:o4-mini → 1188.1
   ExclusivityParticlesLLMStrategy:phi-4-multimodal-instruct → 784.8
   ExclusivityParticlesLLMStrategy:qwen → 782.6
   ExclusivityParticlesLLMStrategy:qwq → 1118.5

SuperplyPuzzle:
 [easy]
   SuperplyCustomStrategy → 928.2
   SuperplyLLMStrategy:deepseek-chat → 895.4
   SuperplyLLMStrategy:deepseek-reasoner → 1285.6
   SuperplyLLMStrategy:gemini-2.5-pro-preview-03-25 → 1133.0
   SuperplyLLMStrategy:gemma → 787.4
   SuperplyLLMStrategy:gpt-4.1 → 1182.9
   SuperplyLLMStrategy:grok-3-mini-beta → 1168.9
   SuperplyLLMStrategy:llama → 747.1
   SuperplyLLMStrategy:o4-mini → 1236.2
   SuperplyLLMStrategy:phi-4-multimodal-instruct → 718.3
   SuperplyLLMStrategy:qwen → 698.0
   SuperplyLLMStrategy:qwq → 1219.1
 [normal]
   SuperplyCustomStrategy → 915.8
   SuperplyLLMStrategy:deepseek-chat → 1013.1
   SuperplyLLMStrategy:deepseek-reasoner → 1222.4
   SuperplyLLMStrategy:gemini-2.5-pro-preview-03-25 → 952.4
   SuperplyLLMStrategy:gemma → 722.3
   SuperplyLLMStrategy:gpt-4.1 → 1173.9
   SuperplyLLMStrategy:grok-3-mini-beta → 1137.7
   SuperplyLLMStrategy:llama → 799.3
   SuperplyLLMStrategy:o4-mini → 1267.8
   SuperplyLLMStrategy:phi-4-multimodal-instruct → 850.1
   SuperplyLLMStrategy:qwen → 772.9
   SuperplyLLMStrategy:qwq → 1172.4

SudoKillMPuzzle:
 [easy]
   SudoKillMCustomStrategy → 1264.9
   SudoKillMLLMStrategy:gemini-2.5-pro-preview-03-25 → 937.8
   SudoKillMLLMStrategy:gemma → 877.6
   SudoKillMLLMStrategy:gpt-4.1 → 1004.3
   SudoKillMLLMStrategy:o4-mini → 1192.9
   SudoKillMLLMStrategy:phi-4-multimodal-instruct → 894.6
   SudoKillMLLMStrategy:qwen → 827.8
 [normal]
   SudoKillMCustomStrategy → 1312.1
   SudoKillMLLMStrategy:gemini-2.5-pro-preview-03-25 → 1009.8
   SudoKillMLLMStrategy:gemma → 911.0
   SudoKillMLLMStrategy:gpt-4.1 → 941.2
   SudoKillMLLMStrategy:o4-mini → 1090.5
   SudoKillMLLMStrategy:phi-4-multimodal-instruct → 964.3
   SudoKillMLLMStrategy:qwen → 771.2

SuperplyMPuzzle:
 [easy]
   SuperplyMCustomStrategy → 1058.9
   SuperplyMLLMStrategy:gemini-2.5-pro-preview-03-25 → 856.0
   SuperplyMLLMStrategy:gemma → 833.7
   SuperplyMLLMStrategy:gpt-4.1 → 1142.3
   SuperplyMLLMStrategy:o4-mini → 1313.6
   SuperplyMLLMStrategy:phi-4-multimodal-instruct → 947.5
   SuperplyMLLMStrategy:qwen → 848.0
 [normal]
   SuperplyMCustomStrategy → 1018.6
   SuperplyMLLMStrategy:gemini-2.5-pro-preview-03-25 → 848.7
   SuperplyMLLMStrategy:gemma → 834.7
   SuperplyMLLMStrategy:gpt-4.1 → 1127.2
   SuperplyMLLMStrategy:o4-mini → 1304.4
   SuperplyMLLMStrategy:phi-4-multimodal-instruct → 960.2
   SuperplyMLLMStrategy:qwen → 906.2

   
